Observability Analysis and Online Calibration of Visual-Inertial-Wheel Odometry for 4WIS4WID Mobile Robots

In this paper, we present a visual-inertial-wheel odometry (VIWO) framework with online calibration for four-wheel independently steered and driven (4WIS4WID) mobile robots. We derive a 2D odometry model directly from the four driving velocities and steering angles, using both the longitudinal rolling constraints and the lateral no-slip constraints of all wheels. A preintegration model and analytical Jacobians are developed for efficient filtering and calibration. An observability analysis of the linearized VIWO system shows that a drive-only model makes all steering offsets unobservable, whereas the proposed redundant model restores their observability. The analysis also identifies four standard VINS unobservable directions and three additional directions associated with the arbitrary placement of the odometry reference frame. Furthermore, we characterize several degenerate motions, including zero yaw rate, constant steering, and a non-rolling wheel, and derive the corresponding excitation conditions for the thirteen wheel intrinsics that remain after fixing the odometry frame reference. The performance of the proposed system has been demonstrated in both simulation and real-world experiments on a 4WIS4WID mobile robot.

==> experimental_paper/table_calibration.tex <==
% Generated by scripts/make_paper_tables.py -- do not edit by hand.
% source: 05 OUTPUT/experiments_slam / paper_run_2 / viwo_accurate_calib
\begin{table}[t]
  \centering
  \caption{Values of the calibration parameters before and after online
    calibration, for \texttt{viwo\_accurate\_calib} on \texttt{paper\_run\_2}. ``Before'' is the marker-derived and
    nominal initialisation the filter starts from; ``after'' is the converged
    estimate at the end of the run. The gauge-fixed wheel is held by construction and
    so has no entry.}
  \label{tab:calibration_table}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Parameter} & \textbf{Before} & \textbf{After} \\
    \midrule
    wheel radii $r$ [m] & [0.0255, 0.0256, 0.0256, 0.0256] & [0.0263, 0.0263, 0.0281, 0.0268] \\
    wheel positions $x_w$ [m] & [-0.1125, -0.1125, 0.1125] & [-0.1029, -0.1029, 0.1454] \\
    wheel positions $y_w$ [m] & [0.1125, -0.1125, -0.1125] & [0.1267, -0.1216, -0.1216] \\
    steering offsets $\delta_o$ [rad] & [0.0086, 0.0065, 0.0127] & [0.0168, -0.0098, -0.0633] \\
    Ext. Pos [m] & [0.1457, 0.0279, 0.0576] & [0.1696, 0.0192, 0.0244] \\
    Ext. Ori [rad] & [1.2085, 1.2093, 1.2091] & [1.2498, 1.2060, 1.2206] \\
    Time offset [s] & 0.00000 & -0.00656 \\
    \bottomrule
  \end{tabular}
\end{table}


==> experimental_paper/table_rpe.tex <==
% Generated by scripts/make_paper_tables.py -- do not edit by hand.
% source: 05 OUTPUT/experiments_slam / paper_run_2
\begin{table}[t]
  \centering
  \caption{Relative pose error (RPE) of each algorithm, as
    degree\,/\,metre over segments of
    2, 5, 10~m of travelled distance. Segment lengths
    are set by the trajectory: the ground-truth path is 26.96~m, so the
    50/100/200~m segments used for driving datasets contain no samples. The metre
    Wheel odometry alone is not listed: it does not measure the vertical channel, so
    a 3D relative error over it reports the length of the run. The last column is the mean normalised innovation squared of the wheel update against
    its own dimension, which should be comparable to it; absolute pose NEES is
    deliberately not reported, because the global position and yaw are the navigation
    frame's gauge and a NEES over them measures a frame convention rather than the
    filter.}
  \label{tab:rpe}
  \begin{tabular}{lcccc}
    \toprule
     & \textbf{2m} & \textbf{5m} & \textbf{10m} & \textbf{wheel NIS} \\
    \midrule
    VIO & 2.917 / 0.401 & 3.848 / 0.623 & 3.370 / 0.813 & -- \\
    true w. cal & 2.381 / 0.148 & 2.539 / 0.195 & 2.840 / 0.203 & 1.52 / 3 \\
    true wo. cal & 2.545 / 0.112 & 3.046 / 0.210 & 3.653 / 0.333 & 2.50 / 3 \\
    bad w. cal & 2.203 / 0.137 & 2.311 / 0.188 & 2.280 / 0.191 & 1.45 / 3 \\
    bad wo. cal & 2.582 / 0.161 & 2.755 / 0.268 & 2.725 / 0.421 & 3.51 / 3 \\
    \bottomrule
  \end{tabular}
\end{table}


==> fig_kinematics_body.tex <==
% =====================================================================
% fig_kinematics_body.tex
% Shared TikZ drawing for the 4WIS4WID kinematic-model figure (Fig. 1).
% \input this file *inside* \begin{document} from both
%   fig_kinematics.tex            (paper figure wrapper)
%   fig_kinematics_standalone.tex (standalone preview wrapper)
% Do NOT \input this from a preamble.
%
% Calling document's preamble must contain:
%   \usepackage{tikz}
%   \usetikzlibrary{calc,arrows.meta,angles,quotes,positioning,patterns}
%
% ---------------------------------------------------------------------
% GEOMETRY NOTES -- edit the numbers below to move things; the arrow /
% label code references only the named coordinates and \deltaN macros,
% so most edits do not require touching the drawing commands.
% ---------------------------------------------------------------------
% Units are bare TikZ units (=1cm at scale 1). The whole picture is
% later rescaled to \columnwidth by the paper wrapper (fig_kinematics.tex)
% via \resizebox, which scales line widths and fonts uniformly along
% with the geometry, so proportions chosen here are what is seen.
%
% All main-panel coordinates below are the "logical" corner positions
% (see ANGLE DERIVATION) uniformly scaled by SCALE = 1.5 relative to the
% frame in which the angles were derived. Scaling every point by the
% same factor changes NO angle (angles are direction-only, scale
% invariant) -- it only opens up extra clearance around wheel 1's dense
% annotation and the {O}/{I}/{C} cluster, without touching \deltaN. Note
% that per-wheel label offsets and arrow lengths below are NOT expressed
% in these scaled coordinates but as fixed absolute distances, so they
% do not grow with SCALE -- see the w_i/p_i label comment further down.
%
% Chassis: rounded rectangle, half-extents (CHASSIS_A, CHASSIS_B) =
% (3.0, 2.4) = 1.5 * (2.0, 1.6), width:height = 1.25 (matches the
% requested ~2:1.6 aspect ratio).
%
% Wheel centres (numbered counter-clockwise from front-right), inset by
% 1.5 * 0.35 = 0.525 from each chassis edge in the unscaled frame:
%   w1 (front-right) = ( 2.475,  1.875)
%   w2 (front-left)  = (-2.475,  1.875)
%   w3 (rear-left)   = (-2.475, -1.875)
%   w4 (rear-right)  = ( 2.475, -1.875)
% To move a wheel: edit its \coordinate line AND rerun the (unscaled)
% angle derivation below, then re-multiply by SCALE if you keep scaling.
%
% ICR: c = (-3.45, 0.45) = 1.5 * (-2.3, 0.3) -- outside the chassis,
% up-and-left, close enough to the footprint to give four clearly
% distinct steering angles (and close enough to keep the overall
% drawing's natural width from ballooning well past \columnwidth, which
% would force a large \resizebox downscale and shrink the text). To move
% the ICR, edit \coordinate (c) below AND recompute \deltaN (see
% derivation) using the UNSCALED wheel/ICR positions (scaling does not
% change the angles, so it is simplest to derive angles in the unscaled
% frame and only scale the coordinates).
%
% ---------------------------------------------------------------------
% ANGLE DERIVATION (by-hand arithmetic in the UNSCALED frame, computed
% once numerically and hard-coded as \deltaN below -- NOT evaluated
% live by TikZ, per the task's explicit fallback allowance. If w_i or c
% move, recompute these four numbers and paste them in; perpendicularity
% is then exact by construction, not by eyeballing).
%
%   For rigid-body rotation about the ICR c, the wheel's rolling
%   direction (velocity direction at the contact point) is exactly the
%   tangent to the circle centred at c through w_i, i.e. perpendicular
%   to the radius vector v_i = w_i - c (unscaled positions):
%       phi_i   = atan2(v_i.y, v_i.x)                  [radius angle]
%       delta_i = phi_i + 90 deg, reduced into (-90 deg, 90 deg]
%   (the +180 deg tangent/-tangent ambiguity is irrelevant for a
%   steering angle: a wheel at delta and at delta+180 is the same
%   physical steering configuration).
%
%   wheel1: v=( 3.9500, 0.9500)  |v|=4.0626  phi= 13.523 deg  delta1=-76.477 deg
%   wheel2: v=( 0.6500, 0.9500)  |v|=1.1511  phi= 55.620 deg  delta2=-34.380 deg
%   wheel3: v=( 0.6500,-1.5500)  |v|=1.6808  phi=-67.249 deg  delta3= 22.751 deg
%   wheel4: v=( 3.9500,-1.5500)  |v|=4.2432  phi=-21.425 deg  delta4= 68.575 deg
%
%   Check: phi_2 - delta_2 = 55.620 - (-34.380) = 90.000 deg exactly,
%   confirming wheel 2's axis is exactly perpendicular to the c--w2
%   line; this pair is used below for the drawn right-angle mark
%   (direction toward c from w2 is phi_2+180 = 235.620 deg, direction
%   back along wheel 2's own axis is delta_2+180 = 145.620 deg -- these
%   two differ by exactly 90 deg, which is what the small square marks).
%   Both are pure directions, so they are unaffected by the SCALE factor.
% ---------------------------------------------------------------------

\definecolor{cbgrey}{gray}{0.55}          % chassis fill (at reduced opacity, see below) + all dashed construction/ICR lines
\definecolor{cbaccent}{RGB}{0,114,178}    % Okabe--Ito blue, colourblind-safe; u_1 only

\tikzset{
  chassis/.style      = {rounded corners=8pt, draw=black, line width=0.7pt, fill=cbgrey, fill opacity=0.30},
  minichassis/.style   = {rounded corners=2pt, draw=black, line width=0.5pt, fill=cbgrey, fill opacity=0.30},
  wheelbody/.style     = {rounded corners=1.2pt, draw=black, line width=0.6pt, fill=white},
  posvec/.style        = {-{Latex[length=2.1mm,width=1.5mm]}, line width=0.8pt, draw=black},
  dvec/.style          = {-{Latex[length=2.1mm,width=1.5mm]}, line width=0.9pt, draw=black},
  dperpvec/.style      = {-{Latex[length=1.7mm,width=1.2mm]}, line width=0.7pt, draw=black},
  uvec/.style          = {-{Latex[open,length=2.3mm,width=1.6mm]}, line width=1.0pt, draw=cbaccent},
  framevec/.style      = {-{Latex[length=1.6mm,width=1.1mm]}, line width=0.55pt, draw=black},
  thinline/.style       = {draw=cbgrey, dash pattern=on 2pt off 1.3pt, line width=0.3pt},
  miniwheel/.style      = {draw=black, line width=0.9pt, line cap=round},
}

\begin{tikzpicture}[>=Latex]

% ---- fixed geometry (scaled by 1.5, see notes above) -----------------------
\coordinate (O)  at (0,0);
\coordinate (w1) at (2.475,1.875);
\coordinate (w2) at (-2.475,1.875);
\coordinate (w3) at (-2.475,-1.875);
\coordinate (w4) at (2.475,-1.875);
\coordinate (c)  at (-3.45,0.45);
\coordinate (Iax) at (1.8,-0.35);  % {I} frame origin -- kept away from p_1 / wheel-1 cluster
\coordinate (Cax) at (2.0,-1.2);   % {C} frame origin

% by-hand steering angles, see derivation above (angles are scale invariant)
\def\deltaW{-76.477}  % wheel 1
\def\deltaX{-34.380}  % wheel 2
\def\deltaY{22.751}   % wheel 3
\def\deltaZ{68.575}   % wheel 4

% ---- chassis --------------------------------------------------------------
\draw[chassis] (-3.0,-2.4) rectangle (3.0,2.4);

% ---- ICR construction lines (behind wheels) --------------------------------
\draw[thinline] (c) -- (w1);
\draw[thinline] (c) -- (w2);
\draw[thinline] (c) -- (w3);
\draw[thinline] (c) -- (w4);

\fill (c) circle (1.1pt);
\node[above=2pt, font=\footnotesize] at (c) {$\mathbf{c}$};

% ---- wheels (each an elongated rounded rect, rotated to its delta_i) ------
\begin{scope}[shift={(w1)}, rotate=\deltaW]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}
\begin{scope}[shift={(w2)}, rotate=\deltaX]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}
\begin{scope}[shift={(w3)}, rotate=\deltaY]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}
\begin{scope}[shift={(w4)}, rotate=\deltaZ]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}

% right-angle mark at wheel 2 (c--w2 line is exactly perpendicular to
% wheel 2's own axis; directions 235.620 deg and 145.620 deg from w2, see
% derivation above). Drawn AFTER the wheels so it sits visibly on top of
% wheel 2's body instead of being hidden under it.
\draw[line width=0.3pt]
  ($(w2)+(235.620:0.26)$) -- ($(w2)+(235.620:0.26)+(145.620:0.26)$) -- ($(w2)+(145.620:0.26)$);

% ---- wheel 1: full annotation ---------------------------------------------
% delta_1 arc, measured from the body x-direction (angle 0) to d_1 (angle
% \deltaW), drawn in the GLOBAL (unrotated) frame centred at w1. Radius
% kept small (0.3) because w1 sits close to the chassis's right edge
% (clearance 0.525) -- a larger radius would cross the boundary.
\draw[thinline] (w1) -- ++(0:0.3);
\draw[line width=0.35pt] ($(w1)+(0:0.3)$) arc[start angle=0, end angle=\deltaW, radius=0.3];
\node[font=\footnotesize] at ($(w1)+(-55:0.5)$) {$\delta_1$};

% d_1, d_1^perp, u_1 and the no-slip decomposition, drawn in wheel 1's own
% (rotated) frame: local +x = d_1 direction. d_1^perp is drawn along LOCAL
% -y (not +y): local +y maps to global direction (0.98,0.18), i.e. almost
% straight toward the nearby right edge (w1's clearance there is only
% 0.525), which is what overflowed the chassis boundary; local -y maps to
% global (-0.98,-0.18), into the open chassis interior, with no loss of
% meaning since "the" perpendicular direction is a sign choice either way.
% u_1 and the decomposition are drawn on the same (-y) side for consistency.
% Node text is NOT rotated by the scope (TikZ only rotates the canvas, not
% node shapes, unless "transform shape" is given -- so labels stay upright).
\begin{scope}[shift={(w1)}, rotate=\deltaW]
  \draw[dvec]     (0,0) -- (1.0,0)    node[right, font=\footnotesize] {$\mathbf{d}_1$};
  % shorter than before (0.42, not 0.6) so it does not reach as far into
  % the interior and stays clear of the p_1 arrow, which passes nearby
  \draw[dperpvec] (0,0) -- (0,-0.42)  node[left, font=\footnotesize] {$\mathbf{d}_1^{\perp}$};
  % u_1 deliberately a few degrees off the d_1 axis so the decomposition is visible
  \draw[uvec] (0,0) -- (0.95,-0.16) node[below right, font=\footnotesize, text=cbaccent] {$\mathbf{u}_1$};
  % dashed parallelogram construction dropping the tip of u_1 onto each axis
  \draw[thinline] (0.95,-0.16) -- (0.95,0);
  \draw[thinline] (0.95,-0.16) -- (0,-0.16);
  \node[above, font=\scriptsize] at (0.95,0)  {$v_1$};
  % Named (not labelled in place): the foot of this component sits inside
  % the wheel body's own footprint (half-width 0.16, so this point is on
  % its edge) AND on the d_1^perp ray, so no nearby anchor/nudge clears
  % the wheel, the arrow and the p_1 line all at once (checked against all
  % three explicitly -- every offset that clears one lands on another).
  % \coordinate still picks up the scope's shift+rotate, so it can be
  % referenced by its GLOBAL position once outside the scope.
  \coordinate (u1dropperp) at (0,-0.16);
\end{scope}
% "=0 (no slip)" callout: a short leader from u1dropperp out to (1.55,2.05),
% the one pocket of open space in this corner (above the p_1 line, left of
% the d_1^perp label, well below the chassis top edge) -- verified clear of
% the wheel body, the p_1 line, and the d_1^perp label by direct coordinate
% check. Re-verify this pocket by eye if the ICR (hence \deltaW) changes.
\draw[thinline] (u1dropperp) -- (1.55,2.05);
\node[left, font=\scriptsize] at (1.55,2.05) {$=0$ (no slip)};

% w_i / p_i labels: placed along each wheel's OWN forward axis direction
% (w2,w3,w4: \deltaX/\deltaY/\deltaZ) or backward direction (w1: \deltaW+180),
% at radius BEYOND the wheel's own half-length (0.5) so the label never
% lands on top of that wheel's own rotated body, regardless of its
% steering angle (a fixed compass anchor like "above left" does not have
% that guarantee once the wheel is rotated -- nor does a radius inside
% 0.5, since the wheel body is centred on this same axis). w1 uses the
% backward direction specifically because its forward direction is
% already used by the d_1/u_1 annotation.
\node[font=\footnotesize] at ($(w1)+(103.523:0.68)$) {$w_1$};

% ---- position vectors -------------------------------------------------------
\draw[posvec] (O) -- ($(O)!0.84!(w1)$) node[midway, above left, font=\footnotesize] {$\mathbf{p}_1$};
\node[font=\footnotesize] at ($(w2)+(\deltaX:0.65)$) {$w_2$};
\node[font=\footnotesize] at ($(w3)+(\deltaY:0.65)$) {$w_3$};
% wheel 4's forward direction points toward the {I}/{C} frame cluster, so
% its label needs extra radius to clear the {C} frame's x-axis arrow, but
% not so much that it closes the gap to p_4 below
\node[font=\footnotesize, yshift=3pt] at ($(w4)+(\deltaZ:0.8)$) {$w_4$};
% p2..p4: labels only (no arrows drawn, to avoid clutter), further out
% along the same direction so they stack radially past w_i without overlap
\node[font=\footnotesize] at ($(w2)+(\deltaX:1.15)$) {$\mathbf{p}_2$};
\node[font=\footnotesize] at ($(w3)+(\deltaY:1.15)$) {$\mathbf{p}_3$};
\node[font=\footnotesize] at ($(w4)+(\deltaZ:1.1)$) {$\mathbf{p}_4$};

% ---- {O}, {I}, {C} frames ---------------------------------------------------
\fill (O) circle (1.1pt);
\draw[framevec] (O) -- ++(0.55,0) node[right, font=\footnotesize] {$x$};
\draw[framevec] (O) -- ++(0,0.55) node[above, font=\footnotesize] {$y$};
\node[below left=1pt and 1pt, font=\footnotesize] at (O) {$\{O\}$};

\fill (Iax) circle (0.9pt);
\draw[framevec] (Iax) -- ++(0.32,0) node[right, font=\scriptsize] {$x$};
\draw[framevec] (Iax) -- ++(0,0.32) node[above, font=\scriptsize] {$y$};
\node[below left=1pt and 1pt, font=\footnotesize] at (Iax) {$\{I\}$};

\fill (Cax) circle (0.9pt);
\draw[framevec] (Cax) -- ++(0.32,0) node[right, font=\scriptsize] {$x$};
\draw[framevec] (Cax) -- ++(0,0.32) node[above, font=\scriptsize] {$y$};
\node[below=6pt, font=\footnotesize] at (Cax) {$\{C\}$};

\draw[posvec] (O) -- ($(O)!0.82!(Iax)$)
  node[midway, below, sloped, font=\footnotesize] {${}^O\mathbf{p}_I$};

% =============================================================================
% INSET PANEL: three miniature ICR-placement sketches, stacked vertically,
% to the right of the main panel (main panel's rightmost extent is the
% chassis edge at x=3.0, with w_4/p_4's labels reaching to about x~2.95,
% so the inset column starts at x=4.6 to leave a clear gap).
% Mini chassis half-extents (MA,MB) = (0.42,0.35); wheel marks are short
% thick segments at the four corners, rotated to an illustrative (not
% calc-derived -- these are schematic only) steering angle. Slot centres
% are 2.3 apart in y.
% =============================================================================
\node[font=\small] at (4.6,3.1) {ICR placement};

% -- (a) ICR far outside the footprint: near-straight driving ---------------
\begin{scope}[shift={(4.6,2.0)}]
  \draw[minichassis] (-0.42,-0.35) rectangle (0.42,0.35);
  \begin{scope}[shift={(0.34,0.27)},  rotate=4]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,0.27)}, rotate=-3] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,-0.27)},rotate=3]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(0.34,-0.27)}, rotate=-4] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  % ICR cross, placed just above the footprint (with a clear gap below the
  % "ICR placement" heading) to read as "far away"
  \draw[line width=0.4pt] (-0.06,0.46) -- (0.06,0.58);
  \draw[line width=0.4pt] (-0.06,0.58) -- (0.06,0.46);
  \node[font=\scriptsize] at (0,-0.62) {(a) ICR far outside};
\end{scope}

% -- (b) ICR inside the footprint: tight turn / spin -------------------------
\begin{scope}[shift={(4.6,-0.3)}]
  \draw[minichassis] (-0.42,-0.35) rectangle (0.42,0.35);
  % point-turn pattern: each wheel axis tangential to the centre (180-deg
  % rotational symmetry, opposite corners share the same angle)
  \begin{scope}[shift={(0.34,0.27)},  rotate=-53] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,0.27)}, rotate=53]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,-0.27)},rotate=-53] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(0.34,-0.27)}, rotate=53]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  % ICR cross at the centre
  \draw[line width=0.4pt] (-0.09,-0.09) -- (0.09,0.09);
  \draw[line width=0.4pt] (-0.09,0.09) -- (0.09,-0.09);
  \node[font=\scriptsize] at (0,-0.62) {(b) ICR inside footprint};
\end{scope}

% -- (c) ICR at infinity: crab (all wheels parallel) --------------------------
\begin{scope}[shift={(4.6,-2.6)}]
  \draw[minichassis] (-0.42,-0.35) rectangle (0.42,0.35);
  \begin{scope}[shift={(0.34,0.27)},  rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,0.27)}, rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,-0.27)},rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(0.34,-0.27)}, rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  % small arrow indicating direction of travel instead of an ICR cross
  \draw[-{Latex[length=1.6mm,width=1.1mm]}, line width=0.6pt] (0,0) -- ++(25:0.42);
  \node[font=\scriptsize] at (0,-0.62) {(c) ICR at infinity (crab)};
\end{scope}

\end{tikzpicture}


==> icra_2027_paper_short/fig_kinematics.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=252.0pt]{fig_kinematics_real.pdf}
  \caption{4WIS4WID mobile robot where each wheel $i$ is
  independently steered by $\delta_i$ and driven at $\omega_{d_i}$, so the
ICR may be placed anywhere in
  the plane.}
  \label{fig:kinematics}
\end{figure}


==> icra_2027_paper_short/fig_kinematics_body.tex <==
% =====================================================================
% fig_kinematics_body.tex
% Shared TikZ drawing for the 4WIS4WID kinematic-model figure (Fig. 1).
% \input this file *inside* \begin{document} from both
%   fig_kinematics.tex            (paper figure wrapper)
%   fig_kinematics_standalone.tex (standalone preview wrapper)
% Do NOT \input this from a preamble.
%
% Calling document's preamble must contain:
%   \usepackage{tikz}
%   \usetikzlibrary{calc,arrows.meta,angles,quotes,positioning,patterns}
%
% ---------------------------------------------------------------------
% GEOMETRY NOTES -- edit the numbers below to move things; the arrow /
% label code references only the named coordinates and \deltaN macros,
% so most edits do not require touching the drawing commands.
% ---------------------------------------------------------------------
% Units are bare TikZ units (=1cm at scale 1). The whole picture is
% later rescaled to \columnwidth by the paper wrapper (fig_kinematics.tex)
% via \resizebox, which scales line widths and fonts uniformly along
% with the geometry, so proportions chosen here are what is seen.
%
% All main-panel coordinates below are the "logical" corner positions
% (see ANGLE DERIVATION) uniformly scaled by SCALE = 1.5 relative to the
% frame in which the angles were derived. Scaling every point by the
% same factor changes NO angle (angles are direction-only, scale
% invariant) -- it only opens up extra clearance around wheel 1's dense
% annotation and the {O}/{I}/{C} cluster, without touching \deltaN. Note
% that per-wheel label offsets and arrow lengths below are NOT expressed
% in these scaled coordinates but as fixed absolute distances, so they
% do not grow with SCALE -- see the w_i/p_i label comment further down.
%
% Chassis: rounded rectangle, half-extents (CHASSIS_A, CHASSIS_B) =
% (3.0, 2.4) = 1.5 * (2.0, 1.6), width:height = 1.25 (matches the
% requested ~2:1.6 aspect ratio).
%
% Wheel centres (numbered counter-clockwise from front-right), inset by
% 1.5 * 0.35 = 0.525 from each chassis edge in the unscaled frame:
%   w1 (front-right) = ( 2.475,  1.875)
%   w2 (front-left)  = (-2.475,  1.875)
%   w3 (rear-left)   = (-2.475, -1.875)
%   w4 (rear-right)  = ( 2.475, -1.875)
% To move a wheel: edit its \coordinate line AND rerun the (unscaled)
% angle derivation below, then re-multiply by SCALE if you keep scaling.
%
% ICR: c = (-3.45, 0.45) = 1.5 * (-2.3, 0.3) -- outside the chassis,
% up-and-left, close enough to the footprint to give four clearly
% distinct steering angles (and close enough to keep the overall
% drawing's natural width from ballooning well past \columnwidth, which
% would force a large \resizebox downscale and shrink the text). To move
% the ICR, edit \coordinate (c) below AND recompute \deltaN (see
% derivation) using the UNSCALED wheel/ICR positions (scaling does not
% change the angles, so it is simplest to derive angles in the unscaled
% frame and only scale the coordinates).
%
% ---------------------------------------------------------------------
% ANGLE DERIVATION (by-hand arithmetic in the UNSCALED frame, computed
% once numerically and hard-coded as \deltaN below -- NOT evaluated
% live by TikZ, per the task's explicit fallback allowance. If w_i or c
% move, recompute these four numbers and paste them in; perpendicularity
% is then exact by construction, not by eyeballing).
%
%   For rigid-body rotation about the ICR c, the wheel's rolling
%   direction (velocity direction at the contact point) is exactly the
%   tangent to the circle centred at c through w_i, i.e. perpendicular
%   to the radius vector v_i = w_i - c (unscaled positions):
%       phi_i   = atan2(v_i.y, v_i.x)                  [radius angle]
%       delta_i = phi_i + 90 deg, reduced into (-90 deg, 90 deg]
%   (the +180 deg tangent/-tangent ambiguity is irrelevant for a
%   steering angle: a wheel at delta and at delta+180 is the same
%   physical steering configuration).
%
%   wheel1: v=( 3.9500, 0.9500)  |v|=4.0626  phi= 13.523 deg  delta1=-76.477 deg
%   wheel2: v=( 0.6500, 0.9500)  |v|=1.1511  phi= 55.620 deg  delta2=-34.380 deg
%   wheel3: v=( 0.6500,-1.5500)  |v|=1.6808  phi=-67.249 deg  delta3= 22.751 deg
%   wheel4: v=( 3.9500,-1.5500)  |v|=4.2432  phi=-21.425 deg  delta4= 68.575 deg
%
%   Check: phi_2 - delta_2 = 55.620 - (-34.380) = 90.000 deg exactly,
%   confirming wheel 2's axis is exactly perpendicular to the c--w2
%   line; this pair is used below for the drawn right-angle mark
%   (direction toward c from w2 is phi_2+180 = 235.620 deg, direction
%   back along wheel 2's own axis is delta_2+180 = 145.620 deg -- these
%   two differ by exactly 90 deg, which is what the small square marks).
%   Both are pure directions, so they are unaffected by the SCALE factor.
% ---------------------------------------------------------------------

\definecolor{cbgrey}{gray}{0.55}          % chassis fill (at reduced opacity, see below) + all dashed construction/ICR lines
\definecolor{cbaccent}{RGB}{0,114,178}    % Okabe--Ito blue, colourblind-safe; u_1 only

\tikzset{
  chassis/.style      = {rounded corners=8pt, draw=black, line width=0.7pt, fill=cbgrey, fill opacity=0.30},
  minichassis/.style   = {rounded corners=2pt, draw=black, line width=0.5pt, fill=cbgrey, fill opacity=0.30},
  wheelbody/.style     = {rounded corners=1.2pt, draw=black, line width=0.6pt, fill=white},
  posvec/.style        = {-{Latex[length=2.1mm,width=1.5mm]}, line width=0.8pt, draw=black},
  dvec/.style          = {-{Latex[length=2.1mm,width=1.5mm]}, line width=0.9pt, draw=black},
  dperpvec/.style      = {-{Latex[length=1.7mm,width=1.2mm]}, line width=0.7pt, draw=black},
  uvec/.style          = {-{Latex[open,length=2.3mm,width=1.6mm]}, line width=1.0pt, draw=cbaccent},
  framevec/.style      = {-{Latex[length=1.6mm,width=1.1mm]}, line width=0.55pt, draw=black},
  thinline/.style       = {draw=cbgrey, dash pattern=on 2pt off 1.3pt, line width=0.3pt},
  miniwheel/.style      = {draw=black, line width=0.9pt, line cap=round},
}

\begin{tikzpicture}[>=Latex]

% ---- fixed geometry (scaled by 1.5, see notes above) -----------------------
\coordinate (O)  at (0,0);
\coordinate (w1) at (2.475,1.875);
\coordinate (w2) at (-2.475,1.875);
\coordinate (w3) at (-2.475,-1.875);
\coordinate (w4) at (2.475,-1.875);
\coordinate (c)  at (-3.45,0.45);
\coordinate (Iax) at (1.8,-0.35);  % {I} frame origin -- kept away from p_1 / wheel-1 cluster
\coordinate (Cax) at (2.0,-1.2);   % {C} frame origin

% by-hand steering angles, see derivation above (angles are scale invariant)
\def\deltaW{-76.477}  % wheel 1
\def\deltaX{-34.380}  % wheel 2
\def\deltaY{22.751}   % wheel 3
\def\deltaZ{68.575}   % wheel 4

% ---- chassis --------------------------------------------------------------
\draw[chassis] (-3.0,-2.4) rectangle (3.0,2.4);

% ---- ICR construction lines (behind wheels) --------------------------------
\draw[thinline] (c) -- (w1);
\draw[thinline] (c) -- (w2);
\draw[thinline] (c) -- (w3);
\draw[thinline] (c) -- (w4);

\fill (c) circle (1.1pt);
\node[above=2pt, font=\footnotesize] at (c) {$\mathbf{c}$};

% ---- wheels (each an elongated rounded rect, rotated to its delta_i) ------
\begin{scope}[shift={(w1)}, rotate=\deltaW]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}
\begin{scope}[shift={(w2)}, rotate=\deltaX]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}
\begin{scope}[shift={(w3)}, rotate=\deltaY]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}
\begin{scope}[shift={(w4)}, rotate=\deltaZ]
  \draw[wheelbody] (-0.5,-0.16) rectangle (0.5,0.16);
\end{scope}

% right-angle mark at wheel 2 (c--w2 line is exactly perpendicular to
% wheel 2's own axis; directions 235.620 deg and 145.620 deg from w2, see
% derivation above). Drawn AFTER the wheels so it sits visibly on top of
% wheel 2's body instead of being hidden under it.
\draw[line width=0.3pt]
  ($(w2)+(235.620:0.26)$) -- ($(w2)+(235.620:0.26)+(145.620:0.26)$) -- ($(w2)+(145.620:0.26)$);

% ---- wheel 1: full annotation ---------------------------------------------
% delta_1 arc, measured from the body x-direction (angle 0) to d_1 (angle
% \deltaW), drawn in the GLOBAL (unrotated) frame centred at w1. Radius
% kept small (0.3) because w1 sits close to the chassis's right edge
% (clearance 0.525) -- a larger radius would cross the boundary.
\draw[thinline] (w1) -- ++(0:0.3);
\draw[line width=0.35pt] ($(w1)+(0:0.3)$) arc[start angle=0, end angle=\deltaW, radius=0.3];
\node[font=\footnotesize] at ($(w1)+(-55:0.5)$) {$\delta_1$};

% d_1, d_1^perp, u_1 and the no-slip decomposition, drawn in wheel 1's own
% (rotated) frame: local +x = d_1 direction. d_1^perp is drawn along LOCAL
% -y (not +y): local +y maps to global direction (0.98,0.18), i.e. almost
% straight toward the nearby right edge (w1's clearance there is only
% 0.525), which is what overflowed the chassis boundary; local -y maps to
% global (-0.98,-0.18), into the open chassis interior, with no loss of
% meaning since "the" perpendicular direction is a sign choice either way.
% u_1 and the decomposition are drawn on the same (-y) side for consistency.
% Node text is NOT rotated by the scope (TikZ only rotates the canvas, not
% node shapes, unless "transform shape" is given -- so labels stay upright).
\begin{scope}[shift={(w1)}, rotate=\deltaW]
  \draw[dvec]     (0,0) -- (1.0,0)    node[right, font=\footnotesize] {$\mathbf{d}_1$};
  % shorter than before (0.42, not 0.6) so it does not reach as far into
  % the interior and stays clear of the p_1 arrow, which passes nearby
  \draw[dperpvec] (0,0) -- (0,-0.42)  node[left, font=\footnotesize] {$\mathbf{d}_1^{\perp}$};
  % u_1 deliberately a few degrees off the d_1 axis so the decomposition is visible
  \draw[uvec] (0,0) -- (0.95,-0.16) node[below right, font=\footnotesize, text=cbaccent] {$\mathbf{u}_1$};
  % dashed parallelogram construction dropping the tip of u_1 onto each axis
  \draw[thinline] (0.95,-0.16) -- (0.95,0);
  \draw[thinline] (0.95,-0.16) -- (0,-0.16);
  \node[above, font=\scriptsize] at (0.95,0)  {$v_1$};
  % Named (not labelled in place): the foot of this component sits inside
  % the wheel body's own footprint (half-width 0.16, so this point is on
  % its edge) AND on the d_1^perp ray, so no nearby anchor/nudge clears
  % the wheel, the arrow and the p_1 line all at once (checked against all
  % three explicitly -- every offset that clears one lands on another).
  % \coordinate still picks up the scope's shift+rotate, so it can be
  % referenced by its GLOBAL position once outside the scope.
  \coordinate (u1dropperp) at (0,-0.16);
\end{scope}
% "=0 (no slip)" callout: a short leader from u1dropperp out to (1.55,2.05),
% the one pocket of open space in this corner (above the p_1 line, left of
% the d_1^perp label, well below the chassis top edge) -- verified clear of
% the wheel body, the p_1 line, and the d_1^perp label by direct coordinate
% check. Re-verify this pocket by eye if the ICR (hence \deltaW) changes.
\draw[thinline] (u1dropperp) -- (1.55,2.05);
\node[left, font=\scriptsize] at (1.55,2.05) {$=0$ (no slip)};

% w_i / p_i labels: placed along each wheel's OWN forward axis direction
% (w2,w3,w4: \deltaX/\deltaY/\deltaZ) or backward direction (w1: \deltaW+180),
% at radius BEYOND the wheel's own half-length (0.5) so the label never
% lands on top of that wheel's own rotated body, regardless of its
% steering angle (a fixed compass anchor like "above left" does not have
% that guarantee once the wheel is rotated -- nor does a radius inside
% 0.5, since the wheel body is centred on this same axis). w1 uses the
% backward direction specifically because its forward direction is
% already used by the d_1/u_1 annotation.
\node[font=\footnotesize] at ($(w1)+(103.523:0.68)$) {$w_1$};

% ---- position vectors -------------------------------------------------------
\draw[posvec] (O) -- ($(O)!0.84!(w1)$) node[midway, above left, font=\footnotesize] {$\mathbf{p}_1$};
\node[font=\footnotesize] at ($(w2)+(\deltaX:0.65)$) {$w_2$};
\node[font=\footnotesize] at ($(w3)+(\deltaY:0.65)$) {$w_3$};
% wheel 4's forward direction points toward the {I}/{C} frame cluster, so
% its label needs extra radius to clear the {C} frame's x-axis arrow, but
% not so much that it closes the gap to p_4 below
\node[font=\footnotesize, yshift=3pt] at ($(w4)+(\deltaZ:0.8)$) {$w_4$};
% p2..p4: labels only (no arrows drawn, to avoid clutter), further out
% along the same direction so they stack radially past w_i without overlap
\node[font=\footnotesize] at ($(w2)+(\deltaX:1.15)$) {$\mathbf{p}_2$};
\node[font=\footnotesize] at ($(w3)+(\deltaY:1.15)$) {$\mathbf{p}_3$};
\node[font=\footnotesize] at ($(w4)+(\deltaZ:1.1)$) {$\mathbf{p}_4$};

% ---- {O}, {I}, {C} frames ---------------------------------------------------
\fill (O) circle (1.1pt);
\draw[framevec] (O) -- ++(0.55,0) node[right, font=\footnotesize] {$x$};
\draw[framevec] (O) -- ++(0,0.55) node[above, font=\footnotesize] {$y$};
\node[below left=1pt and 1pt, font=\footnotesize] at (O) {$\{O\}$};

\fill (Iax) circle (0.9pt);
\draw[framevec] (Iax) -- ++(0.32,0) node[right, font=\scriptsize] {$x$};
\draw[framevec] (Iax) -- ++(0,0.32) node[above, font=\scriptsize] {$y$};
\node[below left=1pt and 1pt, font=\footnotesize] at (Iax) {$\{I\}$};

\fill (Cax) circle (0.9pt);
\draw[framevec] (Cax) -- ++(0.32,0) node[right, font=\scriptsize] {$x$};
\draw[framevec] (Cax) -- ++(0,0.32) node[above, font=\scriptsize] {$y$};
\node[below=6pt, font=\footnotesize] at (Cax) {$\{C\}$};

\draw[posvec] (O) -- ($(O)!0.82!(Iax)$)
  node[midway, below, sloped, font=\footnotesize] {${}^O\mathbf{p}_I$};

% =============================================================================
% INSET PANEL: three miniature ICR-placement sketches, stacked vertically,
% to the right of the main panel (main panel's rightmost extent is the
% chassis edge at x=3.0, with w_4/p_4's labels reaching to about x~2.95,
% so the inset column starts at x=4.6 to leave a clear gap).
% Mini chassis half-extents (MA,MB) = (0.42,0.35); wheel marks are short
% thick segments at the four corners, rotated to an illustrative (not
% calc-derived -- these are schematic only) steering angle. Slot centres
% are 2.3 apart in y.
% =============================================================================
\node[font=\small] at (4.6,3.1) {ICR placement};

% -- (a) ICR far outside the footprint: near-straight driving ---------------
\begin{scope}[shift={(4.6,2.0)}]
  \draw[minichassis] (-0.42,-0.35) rectangle (0.42,0.35);
  \begin{scope}[shift={(0.34,0.27)},  rotate=4]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,0.27)}, rotate=-3] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,-0.27)},rotate=3]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(0.34,-0.27)}, rotate=-4] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  % ICR cross, placed just above the footprint (with a clear gap below the
  % "ICR placement" heading) to read as "far away"
  \draw[line width=0.4pt] (-0.06,0.46) -- (0.06,0.58);
  \draw[line width=0.4pt] (-0.06,0.58) -- (0.06,0.46);
  \node[font=\scriptsize] at (0,-0.62) {(a) ICR far outside};
\end{scope}

% -- (b) ICR inside the footprint: tight turn / spin -------------------------
\begin{scope}[shift={(4.6,-0.3)}]
  \draw[minichassis] (-0.42,-0.35) rectangle (0.42,0.35);
  % point-turn pattern: each wheel axis tangential to the centre (180-deg
  % rotational symmetry, opposite corners share the same angle)
  \begin{scope}[shift={(0.34,0.27)},  rotate=-53] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,0.27)}, rotate=53]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,-0.27)},rotate=-53] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(0.34,-0.27)}, rotate=53]  \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  % ICR cross at the centre
  \draw[line width=0.4pt] (-0.09,-0.09) -- (0.09,0.09);
  \draw[line width=0.4pt] (-0.09,0.09) -- (0.09,-0.09);
  \node[font=\scriptsize] at (0,-0.62) {(b) ICR inside footprint};
\end{scope}

% -- (c) ICR at infinity: crab (all wheels parallel) --------------------------
\begin{scope}[shift={(4.6,-2.6)}]
  \draw[minichassis] (-0.42,-0.35) rectangle (0.42,0.35);
  \begin{scope}[shift={(0.34,0.27)},  rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,0.27)}, rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(-0.34,-0.27)},rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  \begin{scope}[shift={(0.34,-0.27)}, rotate=25] \draw[miniwheel] (-0.11,0) -- (0.11,0); \end{scope}
  % small arrow indicating direction of travel instead of an ICR cross
  \draw[-{Latex[length=1.6mm,width=1.1mm]}, line width=0.6pt] (0,0) -- ++(25:0.42);
  \node[font=\scriptsize] at (0,-0.62) {(c) ICR at infinity (crab)};
\end{scope}

\end{tikzpicture}


==> icra_2027_paper_short/sec_simulation.tex <==
\section{Simulation Validation}
\label{sec:simulation}

\subsection{Setup}

The proposed estimator was implemented in a purpose-built Monte-Carlo
simulator that generates IMU, camera and eight-channel wheel-encoder
measurements from a prescribed body twist, together with the corresponding
ground-truth calibration parameters. Key parameters are listed in
Table~\ref{tab:sim_params}. 

The simulated environment provides dense, persistently tracked visual
features, so the visual-inertial channel alone is already well
constrained; the comparison of interest here is therefore between
calibrated and uncalibrated wheel odometry.

Six trajectories are used: the ICR-sweep excitation of
Section~\ref{sec:excitation}; four trajectories corresponding to the
degeneracies of Table~\ref{tab:degenerate_motions} (straight-line, crab,
constant-radius circle, and stationary); and a figure-eight without
independent heading variation, included as a representative
non-degenerate but unstructured trajectory. Following the gauge-fixing
convention of Section~\ref{sec:structural}, $x_{w_1}$, $y_{w_1}$ and
$\delta_{o_1}$ are held at their nominal values throughout.

\subsection{Calibration Convergence}

Fig.~\ref{fig:exp1} shows the estimation errors and $3\sigma$ bounds for six
runs on the ICR-sweep trajectory, each with an independent realisation of the
measurement noise and of the initial calibration perturbation; each run
continues to $120$~s, but the plot is windowed to the first $40$~s, where the
initial convergence transient is visible. All estimated
parameters converge towards their true values within the reported bounds. The
wheel radii converge fastest at first, consistent with
\eqref{eq:Cj}: the radius sensitivity scales with the wheel angular rate
$\omega_{md_j}$ whereas the position sensitivity scales with the body yaw rate
$\omega$, and $\omega_{md_j} \gg \omega$ at the speeds considered; by $120$~s
(beyond the plotted window) the two have contracted to a comparable level
($46$--$70\%$ of initial uncertainty for the radii, $37$--$66\%$ for the
positions).

% Estimation error (solid) and 3-sigma bound (dotted) vs. time, six
% independent Monte-Carlo runs on the ICR-sweep trajectory, for the IMU-odometry
% extrinsic orientation/position and three representative gauge-fixed wheel
% intrinsics ($r_1$, $\delta_{o2}$, $x_{w2}$).
% Each run is 120s; plot windowed to [0,40]s where the transient is visible.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{../filter_sim_output/exp1_convergence_v2.pdf}
  \caption{Estimation error (solid) and $3\sigma$ bound (dotted) for six Monte-Carlo runs along the ICR-sweep trajectory. Shown are the IMU--odometry extrinsics and three representative wheel intrinsics ($r_1$, $\delta_{o2}$, $x_{w2}$). The plot shows the first 40~s to highlight the initial transient.}
  \label{fig:exp1}
\end{figure}

\subsection{Degenerate Motions}

Fig.~\ref{fig:exp2b} validates Lemma~\ref{lem:const_steering} on a
constant-radius circular trajectory. Rather than plotting individual parameter
errors -- the lemma predicts unobservable \emph{combinations}, not individual
parameters -- we project the covariance onto the two predicted null directions
of \eqref{eq:const_steering_null} and onto two directions in their orthogonal
complement. The predicted null directions retain $100\%$ of their
initial uncertainty over the trajectory, while the complement directions
contract to $30$--$47\%$, confirming the predicted null-space
structure.

% Projection of the wheel-2 (r, delta_o, x_w, y_w) covariance block onto the
% two predicted null directions of Lemma 2 (solid) and two directions in their
% orthogonal complement (dashed), sqrt(n^T P n) vs. time, constant-radius
% circle trajectory.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{../filter_sim_output/exp2b_circle_nulldirs_v2.pdf}
  \caption{Projection of the wheel-2 $(r,\delta_o,x_w,y_w)$ covariance block
  onto the two predicted null directions of Lemma~\ref{lem:const_steering}
  (solid) and two directions in their orthogonal complement (dashed),
  $\sqrt{n^\top P n}$ vs.\ time, constant-radius circle trajectory.}
  \label{fig:exp2b}
\end{figure}

Fig.~\ref{fig:exp2a} validates Lemma~\ref{lem:zero_yaw}. Under straight-line
and crab motion, both of which satisfy $\omega \equiv 0$, the $3\sigma$ bounds
of all eight wheel-position parameters remain at their initial values, while
the wheel radii on the ICR-sweep trajectory contract as expected. Under a
stationary platform, all calibration parameters retain their initial
uncertainty, confirming the no-motion case of Table~\ref{tab:degenerate_motions};
this result is omitted for space.

% Left: 3-sigma bounds of all eight gauge-fixed wheel-position parameters
% under straight-line and crab motion (both omega=0); right: 3-sigma bounds of
% the four wheel radii on the ICR-sweep trajectory, for comparison.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{../filter_sim_output/exp2a_degenerate_omega0_v2.pdf}
%   \caption{Left: $3\sigma$ bounds of all eight gauge-fixed wheel-position
%   parameters under straight-line and crab motion (both $\omega=0$); right:
%   $3\sigma$ bounds of the four wheel radii on the ICR-sweep trajectory, for
%   comparison.}
%   \label{fig:exp2a}
% \end{figure}

\subsection{Planar Motion}

Fig.~\ref{fig:planar} reports the extrinsic and temporal calibration under
strictly planar motion, with the roll and pitch excitation removed. Following
the convention of \cite{Lee2020IROS}, only the extrinsics and time offset are
estimated, so that unobservable parameters do not corrupt the remainder through
the covariance. The out-of-plane component of the extrinsic translation
contracts only partially and then plateaus, retaining $21\%$ of its initial
uncertainty at $120$~s against $1\%$ for the in-plane components, reproducing
the planar degeneracy reported in \cite{Lee2020IROS}. The in-plane orientation
components converge approximately three times more slowly than under the
excited trajectory, as planar motion provides weaker geometric constraints on
roll and pitch.

Notably, the extrinsic yaw is the best-constrained orientation component here,
whereas it is the worst-constrained when the wheel intrinsics are
co-estimated. This is a direct consequence of Lemma~\ref{lem:gauge}: with the
wheel geometry held fixed, the $SE(2)$ gauge freedom that couples the
odometry-frame yaw to the wheel array is absent, and the abundant in-plane
rotation constrains the extrinsic yaw directly.

% Estimation error (solid) and 3-sigma bound (dotted) vs. time, six
% independent Monte-Carlo runs on the ICR-sweep trajectory with roll/pitch
% excitation removed (strictly planar motion), for the IMU-odometry extrinsic
% orientation/position; only extrinsics and time offset are estimated.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{../filter_sim_output/exp_planar_v2.pdf}
  \caption{Estimation error (solid) and $3\sigma$ bound (dotted) for six Monte-Carlo runs along the ICR-sweep trajectory under strictly planar motion. Shown are the IMU--odometry extrinsic orientation and position. Each panel is scaled to its converged ($t>5$~s) range.}
  \label{fig:planar}
\end{figure}

\subsection{Necessity of the Lateral Constraints}

Fig.~\ref{fig:exp4} compares the drive-only map $A$ of
Remark~\ref{rem:naive_reduction} against the augmented map $\bar A$, with the
steering offsets estimated in both cases. The distinction is most clearly seen
analytically: evaluated at a representative preintegration interval, the
sensitivity of the preintegrated measurement to the steering offsets,
$\|\partial\mathbf{g}/\partial\bm\delta_o\|$, is between $325$ and $4770$
times smaller under the drive-only map than under the augmented map. This is the
finite-noise counterpart of Lemma~\ref{lem:drive_only}, which establishes that
the corresponding columns of $\mathbf{M}$ vanish identically at the true state;
away from the true state the drive-only model retains a weak second-order
sensitivity through its own residual miscalibration, which decays as the
estimate improves. Consistent with this, the covariance contraction rate of the
drive-only model stalls over the second half of the trajectory
($0.923$ versus $0.787$ for the augmented map on $\delta_{o3}$), indicating that
the apparent reduction in reported uncertainty is not matched by a
corresponding gain in information.

% Top: steering-offset error trajectories (degrees) for the 4-row (drive-only)
% and 8-row (augmented) wheel models, three steering offsets, icr_sweep
% trajectory; bottom: covariance contraction sigma(t)/sigma(0) for the same
% three offsets, showing the drive-only model's second-half stall relative to
% the augmented map.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{../filter_sim_output/exp4_4row_vs_8row_v2.pdf}
%   \caption{Top: steering-offset error trajectories (degrees) for the 4-row
%   (drive-only) and 8-row (augmented) wheel models, three steering offsets,
%   ICR-sweep trajectory; bottom: covariance contraction $\sigma(t)/\sigma(0)$
%   for the same three offsets.}
%   \label{fig:exp4}
% \end{figure}

\subsection{Structural Unobservability and Excitation}

Table~\ref{tab:rank} reports the numerical rank of the accumulated information
matrix $\sum_t \mathbf{H}_t^\top\mathbf{H}_t$, restricted to the thirteen
intrinsics remaining after $SE(2)$ gauge fixing and column-scaled to account
for their differing natural magnitudes. Two observations follow. First, the rank ordering across
trajectories --- ICR sweep, figure-eight, then the three degenerate
trajectories --- confirms quantitatively that trajectory design determines
which parameters are identifiable, and that the ICR-sweep construction of
Section~\ref{sec:excitation} is the best-conditioned of those considered.
Second, the rank is unchanged when the wheel layout is perturbed to a
deliberately asymmetric configuration, and the principal angles between the
unobservable subspaces obtained from ten independent draws of the true
parameters remain below $2.6^\circ$, indicating that the residual
unobservable subspace is a structural property rather than an artefact of the
particular geometry.

\subsection{Estimation Accuracy and Consistency}

Table~\ref{tab:rpe} reports relative pose error and average NEES over
$20$~Monte-Carlo runs for four configurations of initial calibration accuracy
and online calibration. With
accurate initial calibration the estimator performs comparably with and without
online calibration. With perturbed initial values and calibration disabled,
performance degrades catastrophically: relative pose error increases by a
factor of $70$ in rotation and over $8000$ in translation, and NEES by a
factor of $48$, relative to the healthy
configurations. Enabling online calibration recovers essentially all of this
loss, returning the estimator to within $15\%$ of the accurately-initialised
case.

Consistent with the linearised visual-inertial literature, the estimator
exhibits gradual overconfidence in the calibration subspace. Individual updates
remain locally consistent, with mean normalised innovation squared of $0.74$
and $0.86$ per degree of freedom for the wheel and camera channels
respectively (accepted updates only; rejected updates carry NIS values
orders of magnitude higher and would dominate an unfiltered mean), but the
accumulated covariance contracts faster than the
estimation error. This is the known effect of repeated relinearisation against
updated clone poses and would be addressed by an observability-constrained
formulation~\cite{Huang2012, Hesch2014}; as the contribution of this work is
the observability analysis rather than a consistency-improved estimator, we
report it as observed.


==> icra_2027_paper_short/tab_rank.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{Singular-value spectrum of the accumulated, column-scaled information matrix over the 13 intrinsics remaining after $SE(2)$ gauge fixing, for the symmetric and an asymmetric wheel layout. Rank is the count of singular values above $10^{-6}\sigma_1$; condition number is $\sigma_1/\sigma_r$ and gap is $\sigma_r/\sigma_{r+1}$, both evaluated at each row's own rank $r$ -- the boundary separating the informative directions from the structurally unobservable ones.}
\label{tab:rank}
\begin{tabular}{llcp{3.8in}rr}
\toprule
Trajectory & Layout & Rank & Singular values $\sigma_1,\ldots,\sigma_{13}$ (column-scaled) & Cond.\ $\sigma_1/\sigma_r$ & Gap $\sigma_r/\sigma_{r+1}$ \\
\midrule
ICR sweep & sym & 7/13 & 9.3e-1, 7.7e-1, 6.9e-1, 2.1e-1, 9.7e-2, 8.9e-2, 1.7e-2, 9.4e-9, 2.5e-9, 7.8e-10, 2.8e-10, 0, 0 & 5.36e+1 & 1.85e+6 \\
 & asym & 7/13 & 9.4e-1, 8.2e-1, 6.5e-1, 2.1e-1, 9.7e-2, 8.6e-2, 1.7e-2, 7.5e-9, 4.4e-9, 1.8e-9, 0, 0, 0 & 5.41e+1 & 2.32e+6 \\
\addlinespace
Figure-eight & sym & 6/13 & 7.5e-1, 4.4e-1, 1.4e-1, 8.0e-2, 5.0e-2, 1.2e-2, 8.1e-9, 4.9e-9, 1.8e-9, 1.1e-9, 0, 0, 0 & 5.98e+1 & 1.54e+6 \\
 & asym & 6/13 & 7.5e-1, 4.5e-1, 1.4e-1, 7.3e-2, 5.0e-2, 1.2e-2, 3.4e-9, 1.0e-9, 0, 0, 0, 0, 0 & 6.02e+1 & 3.70e+6 \\
\addlinespace
Circle & sym & 3/13 & 9.1e-1, 3.2e-1, 7.1e-2, 6.5e-9, 4.5e-9, 4.2e-9, 2.3e-9, 7.6e-10, 0, 0, 0, 0, 0 & 1.28e+1 & 1.08e+7 \\
 & asym & 3/13 & 8.7e-1, 3.2e-1, 6.8e-2, 7.0e-9, 3.1e-9, 2.3e-9, 1.3e-9, 4.2e-10, 0, 0, 0, 0, 0 & 1.28e+1 & 9.68e+6 \\
\addlinespace
Straight & sym & 3/13 & 1.3e+0, 5.4e-1, 2.3e-2, 2.4e-8, 3.0e-9, 2.4e-10, 1.6e-10, 1.4e-10, 1.3e-10, 1.3e-10, 1.2e-10, 0, 0 & 5.59e+1 & 9.82e+5 \\
 & asym & 3/13 & 1.4e+0, 5.4e-1, 2.3e-2, 1.8e-8, 1.1e-8, 8.7e-10, 2.8e-10, 2.0e-10, 1.6e-10, 1.5e-10, 1.4e-10, 1.2e-10, 1.2e-10 & 5.85e+1 & 1.27e+6 \\
\addlinespace
Crab & sym & 3/13 & 1.2e+0, 4.0e-1, 1.7e-2, 9.4e-9, 1.6e-10, 1.2e-10, 1.1e-10, 9.1e-11, 9.1e-11, 8.7e-11, 0, 0, 0 & 6.66e+1 & 1.85e+6 \\
 & asym & 3/13 & 1.0e+0, 4.0e-1, 1.7e-2, 1.2e-8, 4.2e-10, 1.2e-10, 1.2e-10, 9.8e-11, 9.2e-11, 8.6e-11, 7.8e-11, 0, 0 & 6.00e+1 & 1.39e+6 \\
\addlinespace
\bottomrule
\end{tabular}
\end{table*}


==> icra_2027_paper_short/tab_sim_params.tex <==
\begin{table}[t]
\centering
\small
\caption{Simulation parameters and prior standard deviations}
\label{tab:sim_params}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
\toprule
Parameter & Value & Parameter & Value \\
\midrule
Camera rate & 10~Hz & IMU rate & 200~Hz \\
Wheel encoder rate & 100~Hz & Clones in window & 11 \\
Max features/update & 100 & Pixel noise $\sigma_{px}$ & 1~px \\
Gyro white noise $\sigma_g$ & 0.0001~rad/s & Gyro bias RW $\sigma_{bg}$ & $10^{-5}$~rad/s \\
Accel white noise $\sigma_a$ & 0.0001~m/s$^2$ & Accel bias RW $\sigma_{ba}$ & $10^{-5}$~m/s$^2$ \\
Drive-encoder noise $\sigma_{\omega_d}$ & 0.001~rad/s & Steering-encoder noise $\sigma_\delta$ & 0.001~rad \\
Lateral pseudo-noise $\sigma_{lat}$ & 0.001 & Wheel noise floor $\sigma_\theta,\sigma_{xy}$ & 4.4721e-5~rad, 4.4721e-5~m \\
Perturb: radii (rel.) & 1\% & Perturb: wheel position & 0.01~m \\
Perturb: steering offset & 0.01~rad & Perturb: extrinsic orientation & 0.01~rad \\
Perturb: extrinsic position & 0.1~m & Perturb: time offset & 0.01~s \\
\bottomrule
\end{tabular}%
}
\end{table}


==> icra_2027_paper_short/table_calibration.tex <==
% Generated by scripts/make_paper_tables.py -- do not edit by hand.
% source: 05 OUTPUT/experiments_slam / paper_run_2 / viwo_accurate_calib
\begin{table}[t]
  \centering
  \caption{Values of the calibration parameters before and after online
    calibration, for \texttt{viwo\_accurate\_calib} on \texttt{paper\_run\_2}. ``Before'' is the marker-derived and
    nominal initialisation the filter starts from; ``after'' is the converged
    estimate at the end of the run. The gauge-fixed wheel is held by construction and
    so has no entry.}
  \label{tab:calibration_table}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Parameter} & \textbf{Before} & \textbf{After} \\
    \midrule
    wheel radii $r$ [m] & [0.0255, 0.0256, 0.0256, 0.0256] & [0.0263, 0.0263, 0.0281, 0.0268] \\
    wheel positions $x_w$ [m] & [-0.1125, -0.1125, 0.1125] & [-0.1029, -0.1029, 0.1454] \\
    wheel positions $y_w$ [m] & [0.1125, -0.1125, -0.1125] & [0.1267, -0.1216, -0.1216] \\
    steering offsets $\delta_o$ [rad] & [0.0086, 0.0065, 0.0127] & [0.0168, -0.0098, -0.0633] \\
    Ext. Pos [m] & [0.1457, 0.0279, 0.0576] & [0.1696, 0.0192, 0.0244] \\
    Ext. Ori [rad] & [1.2085, 1.2093, 1.2091] & [1.2498, 1.2060, 1.2206] \\
    Time offset [s] & 0.00000 & -0.00656 \\
    \bottomrule
  \end{tabular}
\end{table}


==> icra_2027_paper_short/table_rpe.tex <==
% Generated by scripts/make_paper_tables.py -- do not edit by hand.
% source: 05 OUTPUT/experiments_slam / paper_run_2
\begin{table}[t]
  \centering
  \caption{Relative pose error (RPE) of each algorithm, as
    degree\,/\,metre over segments of
    2, 5, 10~m of travelled distance. Segment lengths
    are set by the trajectory: the ground-truth path is 26.96~m, so the
    50/100/200~m segments used for driving datasets contain no samples. The metre
    Wheel odometry alone is not listed: it does not measure the vertical channel, so
    a 3D relative error over it reports the length of the run. The last column is the mean normalised innovation squared of the wheel update against
    its own dimension, which should be comparable to it; absolute pose NEES is
    deliberately not reported, because the global position and yaw are the navigation
    frame's gauge and a NEES over them measures a frame convention rather than the
    filter.}
  \label{tab:rpe}
  \begin{tabular}{lcccc}
    \toprule
     & \textbf{2m} & \textbf{5m} & \textbf{10m} & \textbf{wheel NIS} \\
    \midrule
    VIO & 2.917 / 0.401 & 3.848 / 0.623 & 3.370 / 0.813 & -- \\
    true w. cal & 2.381 / 0.148 & 2.539 / 0.195 & 2.840 / 0.203 & 1.52 / 3 \\
    true wo. cal & 2.545 / 0.112 & 3.046 / 0.210 & 3.653 / 0.333 & 2.50 / 3 \\
    bad w. cal & 2.203 / 0.137 & 2.311 / 0.188 & 2.280 / 0.191 & 1.45 / 3 \\
    bad wo. cal & 2.582 / 0.161 & 2.755 / 0.268 & 2.725 / 0.421 & 3.51 / 3 \\
    \bottomrule
  \end{tabular}
\end{table}


==> sec_simulation.tex <==
\section{Simulation Validation}
\label{sec:simulation}

\subsection{Setup}

The proposed estimator was implemented in a purpose-built Monte-Carlo
simulator that generates IMU, camera and eight-channel wheel-encoder
measurements from a prescribed body twist, together with the corresponding
ground-truth calibration parameters. Key parameters are listed in
Table~\ref{tab:sim_params}. 

The simulated environment provides dense, persistently tracked visual
features, so the visual-inertial channel alone is already well
constrained; the comparison of interest here is therefore between
calibrated and uncalibrated wheel odometry.

Six trajectories are used: the ICR-sweep excitation of
Section~\ref{sec:excitation}; four trajectories corresponding to the
degeneracies of Table~\ref{tab:degenerate_motions} (straight-line, crab,
constant-radius circle, and stationary); and a figure-eight without
independent heading variation, included as a representative
non-degenerate but unstructured trajectory. Following the gauge-fixing
convention of Section~\ref{sec:structural}, $x_{w_1}$, $y_{w_1}$ and
$\delta_{o_1}$ are held at their nominal values throughout.

\subsection{Calibration Convergence}

Fig.~\ref{fig:exp1} shows the estimation errors and $3\sigma$ bounds for six
runs on the ICR-sweep trajectory, each with an independent realisation of the
measurement noise and of the initial calibration perturbation; each run
continues to $120$~s, but the plot is windowed to the first $40$~s, where the
initial convergence transient is visible. All estimated
parameters converge towards their true values within the reported bounds. The
wheel radii converge fastest at first, consistent with
\eqref{eq:Cj}: the radius sensitivity scales with the wheel angular rate
$\omega_{md_j}$ whereas the position sensitivity scales with the body yaw rate
$\omega$, and $\omega_{md_j} \gg \omega$ at the speeds considered; by $120$~s
(beyond the plotted window) the two have contracted to a comparable level
($46$--$70\%$ of initial uncertainty for the radii, $37$--$66\%$ for the
positions).

% Estimation error (solid) and 3-sigma bound (dotted) vs. time, six
% independent Monte-Carlo runs on the ICR-sweep trajectory, for the IMU-odometry
% extrinsic orientation/position and three representative gauge-fixed wheel
% intrinsics ($r_1$, $\delta_{o2}$, $x_{w2}$).
% Each run is 120s; plot windowed to [0,40]s where the transient is visible.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{../filter_sim_output/exp1_convergence_v2.pdf}
  \caption{Estimation error (solid) and $3\sigma$ bound (dotted) for six Monte-Carlo runs along the ICR-sweep trajectory. Shown are the IMU--odometry extrinsics and three representative wheel intrinsics ($r_1$, $\delta_{o2}$, $x_{w2}$). The plot shows the first 40~s to highlight the initial transient.}
  \label{fig:exp1}
\end{figure}

\subsection{Degenerate Motions}

Fig.~\ref{fig:exp2b} validates Lemma~\ref{lem:const_steering} on a
constant-radius circular trajectory. Rather than plotting individual parameter
errors -- the lemma predicts unobservable \emph{combinations}, not individual
parameters -- we project the covariance onto the two predicted null directions
of \eqref{eq:const_steering_null} and onto two directions in their orthogonal
complement. The predicted null directions retain $100\%$ of their
initial uncertainty over the trajectory, while the complement directions
contract to $30$--$47\%$, confirming the predicted null-space
structure.

% Projection of the wheel-2 (r, delta_o, x_w, y_w) covariance block onto the
% two predicted null directions of Lemma 2 (solid) and two directions in their
% orthogonal complement (dashed), sqrt(n^T P n) vs. time, constant-radius
% circle trajectory.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{../filter_sim_output/exp2b_circle_nulldirs_v2.pdf}
  \caption{Projection of the wheel-2 $(r,\delta_o,x_w,y_w)$ covariance block
  onto the two predicted null directions of Lemma~\ref{lem:const_steering}
  (solid) and two directions in their orthogonal complement (dashed),
  $\sqrt{n^\top P n}$ vs.\ time, constant-radius circle trajectory.}
  \label{fig:exp2b}
\end{figure}

Fig.~\ref{fig:exp2a} validates Lemma~\ref{lem:zero_yaw}. Under straight-line
and crab motion, both of which satisfy $\omega \equiv 0$, the $3\sigma$ bounds
of all eight wheel-position parameters remain at their initial values, while
the wheel radii on the ICR-sweep trajectory contract as expected. Under a
stationary platform, all calibration parameters retain their initial
uncertainty, confirming the no-motion case of Table~\ref{tab:degenerate_motions};
this result is omitted for space.

% Left: 3-sigma bounds of all eight gauge-fixed wheel-position parameters
% under straight-line and crab motion (both omega=0); right: 3-sigma bounds of
% the four wheel radii on the ICR-sweep trajectory, for comparison.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{../filter_sim_output/exp2a_degenerate_omega0_v2.pdf}
%   \caption{Left: $3\sigma$ bounds of all eight gauge-fixed wheel-position
%   parameters under straight-line and crab motion (both $\omega=0$); right:
%   $3\sigma$ bounds of the four wheel radii on the ICR-sweep trajectory, for
%   comparison.}
%   \label{fig:exp2a}
% \end{figure}

\subsection{Planar Motion}

Fig.~\ref{fig:planar} reports the extrinsic and temporal calibration under
strictly planar motion, with the roll and pitch excitation removed. Following
the convention of \cite{Lee2020IROS}, only the extrinsics and time offset are
estimated, so that unobservable parameters do not corrupt the remainder through
the covariance. The out-of-plane component of the extrinsic translation
contracts only partially and then plateaus, retaining $21\%$ of its initial
uncertainty at $120$~s against $1\%$ for the in-plane components, reproducing
the planar degeneracy reported in \cite{Lee2020IROS}. The in-plane orientation
components converge approximately three times more slowly than under the
excited trajectory, as planar motion provides weaker geometric constraints on
roll and pitch.

Notably, the extrinsic yaw is the best-constrained orientation component here,
whereas it is the worst-constrained when the wheel intrinsics are
co-estimated. This is a direct consequence of Lemma~\ref{lem:gauge}: with the
wheel geometry held fixed, the $SE(2)$ gauge freedom that couples the
odometry-frame yaw to the wheel array is absent, and the abundant in-plane
rotation constrains the extrinsic yaw directly.

% Estimation error (solid) and 3-sigma bound (dotted) vs. time, six
% independent Monte-Carlo runs on the ICR-sweep trajectory with roll/pitch
% excitation removed (strictly planar motion), for the IMU-odometry extrinsic
% orientation/position; only extrinsics and time offset are estimated.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{../filter_sim_output/exp_planar_v2.pdf}
  \caption{Estimation error (solid) and $3\sigma$ bound (dotted) for six Monte-Carlo runs along the ICR-sweep trajectory under strictly planar motion. Shown are the IMU--odometry extrinsic orientation and position. Each panel is scaled to its converged ($t>5$~s) range.}
  \label{fig:planar}
\end{figure}

\subsection{Necessity of the Lateral Constraints}

Fig.~\ref{fig:exp4} compares the drive-only map $A$ of
Remark~\ref{rem:naive_reduction} against the augmented map $\bar A$, with the
steering offsets estimated in both cases. The distinction is most clearly seen
analytically: evaluated at a representative preintegration interval, the
sensitivity of the preintegrated measurement to the steering offsets,
$\|\partial\mathbf{g}/\partial\bm\delta_o\|$, is between $325$ and $4770$
times smaller under the drive-only map than under the augmented map. This is the
finite-noise counterpart of Lemma~\ref{lem:drive_only}, which establishes that
the corresponding columns of $\mathbf{M}$ vanish identically at the true state;
away from the true state the drive-only model retains a weak second-order
sensitivity through its own residual miscalibration, which decays as the
estimate improves. Consistent with this, the covariance contraction rate of the
drive-only model stalls over the second half of the trajectory
($0.923$ versus $0.787$ for the augmented map on $\delta_{o3}$), indicating that
the apparent reduction in reported uncertainty is not matched by a
corresponding gain in information.

% Top: steering-offset error trajectories (degrees) for the 4-row (drive-only)
% and 8-row (augmented) wheel models, three steering offsets, icr_sweep
% trajectory; bottom: covariance contraction sigma(t)/sigma(0) for the same
% three offsets, showing the drive-only model's second-half stall relative to
% the augmented map.
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth]{../filter_sim_output/exp4_4row_vs_8row_v2.pdf}
%   \caption{Top: steering-offset error trajectories (degrees) for the 4-row
%   (drive-only) and 8-row (augmented) wheel models, three steering offsets,
%   ICR-sweep trajectory; bottom: covariance contraction $\sigma(t)/\sigma(0)$
%   for the same three offsets.}
%   \label{fig:exp4}
% \end{figure}

\subsection{Structural Unobservability and Excitation}

Table~\ref{tab:rank} reports the numerical rank of the accumulated information
matrix $\sum_t \mathbf{H}_t^\top\mathbf{H}_t$, restricted to the thirteen
intrinsics remaining after $SE(2)$ gauge fixing and column-scaled to account
for their differing natural magnitudes. Two observations follow. First, the rank ordering across
trajectories --- ICR sweep, figure-eight, then the three degenerate
trajectories --- confirms quantitatively that trajectory design determines
which parameters are identifiable, and that the ICR-sweep construction of
Section~\ref{sec:excitation} is the best-conditioned of those considered.
Second, the rank is unchanged when the wheel layout is perturbed to a
deliberately asymmetric configuration, and the principal angles between the
unobservable subspaces obtained from ten independent draws of the true
parameters remain below $2.6^\circ$, indicating that the residual
unobservable subspace is a structural property rather than an artefact of the
particular geometry.

\subsection{Estimation Accuracy and Consistency}

Table~\ref{tab:rpe} reports relative pose error and average NEES over
$20$~Monte-Carlo runs for four configurations of initial calibration accuracy
and online calibration. With
accurate initial calibration the estimator performs comparably with and without
online calibration. With perturbed initial values and calibration disabled,
performance degrades catastrophically: relative pose error increases by a
factor of $70$ in rotation and over $8000$ in translation, and NEES by a
factor of $48$, relative to the healthy
configurations. Enabling online calibration recovers essentially all of this
loss, returning the estimator to within $15\%$ of the accurately-initialised
case.

Consistent with the linearised visual-inertial literature, the estimator
exhibits gradual overconfidence in the calibration subspace. Individual updates
remain locally consistent, with mean normalised innovation squared of $0.74$
and $0.86$ per degree of freedom for the wheel and camera channels
respectively (accepted updates only; rejected updates carry NIS values
orders of magnitude higher and would dominate an unfiltered mean), but the
accumulated covariance contracts faster than the
estimation error. This is the known effect of repeated relinearisation against
updated clone poses and would be addressed by an observability-constrained
formulation~\cite{Huang2012, Hesch2014}; as the contribution of this work is
the observability analysis rather than a consistency-improved estimator, we
report it as observed.


==> tab_rank.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{Singular-value spectrum of the accumulated, column-scaled information matrix over the 13 intrinsics remaining after $SE(2)$ gauge fixing, for the symmetric and an asymmetric wheel layout. Rank is the count of singular values above $10^{-6}\sigma_1$; condition number is $\sigma_1/\sigma_r$ and gap is $\sigma_r/\sigma_{r+1}$, both evaluated at each row's own rank $r$ -- the boundary separating the informative directions from the structurally unobservable ones.}
\label{tab:rank}
\begin{tabular}{llcp{3.8in}rr}
\toprule
Trajectory & Layout & Rank & Singular values $\sigma_1,\ldots,\sigma_{13}$ (column-scaled) & Cond.\ $\sigma_1/\sigma_r$ & Gap $\sigma_r/\sigma_{r+1}$ \\
\midrule
ICR sweep & sym & 7/13 & 9.3e-1, 7.7e-1, 6.9e-1, 2.1e-1, 9.7e-2, 8.9e-2, 1.7e-2, 9.4e-9, 2.5e-9, 7.8e-10, 2.8e-10, 0, 0 & 5.36e+1 & 1.85e+6 \\
 & asym & 7/13 & 9.4e-1, 8.2e-1, 6.5e-1, 2.1e-1, 9.7e-2, 8.6e-2, 1.7e-2, 7.5e-9, 4.4e-9, 1.8e-9, 0, 0, 0 & 5.41e+1 & 2.32e+6 \\
\addlinespace
Figure-eight & sym & 6/13 & 7.5e-1, 4.4e-1, 1.4e-1, 8.0e-2, 5.0e-2, 1.2e-2, 8.1e-9, 4.9e-9, 1.8e-9, 1.1e-9, 0, 0, 0 & 5.98e+1 & 1.54e+6 \\
 & asym & 6/13 & 7.5e-1, 4.5e-1, 1.4e-1, 7.3e-2, 5.0e-2, 1.2e-2, 3.4e-9, 1.0e-9, 0, 0, 0, 0, 0 & 6.02e+1 & 3.70e+6 \\
\addlinespace
Circle & sym & 3/13 & 9.1e-1, 3.2e-1, 7.1e-2, 6.5e-9, 4.5e-9, 4.2e-9, 2.3e-9, 7.6e-10, 0, 0, 0, 0, 0 & 1.28e+1 & 1.08e+7 \\
 & asym & 3/13 & 8.7e-1, 3.2e-1, 6.8e-2, 7.0e-9, 3.1e-9, 2.3e-9, 1.3e-9, 4.2e-10, 0, 0, 0, 0, 0 & 1.28e+1 & 9.68e+6 \\
\addlinespace
Straight & sym & 3/13 & 1.3e+0, 5.4e-1, 2.3e-2, 2.4e-8, 3.0e-9, 2.4e-10, 1.6e-10, 1.4e-10, 1.3e-10, 1.3e-10, 1.2e-10, 0, 0 & 5.59e+1 & 9.82e+5 \\
 & asym & 3/13 & 1.4e+0, 5.4e-1, 2.3e-2, 1.8e-8, 1.1e-8, 8.7e-10, 2.8e-10, 2.0e-10, 1.6e-10, 1.5e-10, 1.4e-10, 1.2e-10, 1.2e-10 & 5.85e+1 & 1.27e+6 \\
\addlinespace
Crab & sym & 3/13 & 1.2e+0, 4.0e-1, 1.7e-2, 9.4e-9, 1.6e-10, 1.2e-10, 1.1e-10, 9.1e-11, 9.1e-11, 8.7e-11, 0, 0, 0 & 6.66e+1 & 1.85e+6 \\
 & asym & 3/13 & 1.0e+0, 4.0e-1, 1.7e-2, 1.2e-8, 4.2e-10, 1.2e-10, 1.2e-10, 9.8e-11, 9.2e-11, 8.6e-11, 7.8e-11, 0, 0 & 6.00e+1 & 1.39e+6 \\
\addlinespace
\bottomrule
\end{tabular}
\end{table*}


==> tab_sim_params.tex <==
\begin{table}[t]
\centering
\small
\caption{Simulation parameters and prior standard deviations}
\label{tab:sim_params}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
\toprule
Parameter & Value & Parameter & Value \\
\midrule
Camera rate & 10~Hz & IMU rate & 200~Hz \\
Wheel encoder rate & 100~Hz & Clones in window & 11 \\
Max features/update & 100 & Pixel noise $\sigma_{px}$ & 1~px \\
Gyro white noise $\sigma_g$ & 0.0001~rad/s & Gyro bias RW $\sigma_{bg}$ & $10^{-5}$~rad/s \\
Accel white noise $\sigma_a$ & 0.0001~m/s$^2$ & Accel bias RW $\sigma_{ba}$ & $10^{-5}$~m/s$^2$ \\
Drive-encoder noise $\sigma_{\omega_d}$ & 0.001~rad/s & Steering-encoder noise $\sigma_\delta$ & 0.001~rad \\
Lateral pseudo-noise $\sigma_{lat}$ & 0.001 & Wheel noise floor $\sigma_\theta,\sigma_{xy}$ & 4.4721e-5~rad, 4.4721e-5~m \\
Perturb: radii (rel.) & 1\% & Perturb: wheel position & 0.01~m \\
Perturb: steering offset & 0.01~rad & Perturb: extrinsic orientation & 0.01~rad \\
Perturb: extrinsic position & 0.1~m & Perturb: time offset & 0.01~s \\
\bottomrule
\end{tabular}%
}
\end{table}


==> table_calibration.tex <==
% Generated by scripts/make_paper_tables.py -- do not edit by hand.
% source: 05 OUTPUT/experiments_slam / paper_run_2 / viwo_accurate_calib
\begin{table}[t]
  \centering
  \caption{Values of the calibration parameters before and after online
    calibration, for \texttt{viwo\_accurate\_calib} on \texttt{paper\_run\_2}. ``Before'' is the marker-derived and
    nominal initialisation the filter starts from; ``after'' is the converged
    estimate at the end of the run. The gauge-fixed wheel is held by construction and
    so has no entry.}
  \label{tab:calibration_table}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Parameter} & \textbf{Before} & \textbf{After} \\
    \midrule
    wheel radii $r$ [m] & [0.0255, 0.0256, 0.0256, 0.0256] & [0.0263, 0.0263, 0.0281, 0.0268] \\
    wheel positions $x_w$ [m] & [-0.1125, -0.1125, 0.1125] & [-0.1029, -0.1029, 0.1454] \\
    wheel positions $y_w$ [m] & [0.1125, -0.1125, -0.1125] & [0.1267, -0.1216, -0.1216] \\
    steering offsets $\delta_o$ [rad] & [0.0086, 0.0065, 0.0127] & [0.0168, -0.0098, -0.0633] \\
    Ext. Pos [m] & [0.1457, 0.0279, 0.0576] & [0.1696, 0.0192, 0.0244] \\
    Ext. Ori [rad] & [1.2085, 1.2093, 1.2091] & [1.2498, 1.2060, 1.2206] \\
    Time offset [s] & 0.00000 & -0.00656 \\
    \bottomrule
  \end{tabular}
\end{table}


==> table_rpe.tex <==
% Generated by scripts/make_paper_tables.py -- do not edit by hand.
% source: 05 OUTPUT/experiments_slam / paper_run_2
\begin{table}[t]
  \centering
  \caption{Relative pose error (RPE) of each algorithm, as
    degree\,/\,metre over segments of
    2, 5, 10~m of travelled distance. Segment lengths
    are set by the trajectory: the ground-truth path is 26.96~m, so the
    50/100/200~m segments used for driving datasets contain no samples. The metre
    Wheel odometry alone is not listed: it does not measure the vertical channel, so
    a 3D relative error over it reports the length of the run. The last column is the mean normalised innovation squared of the wheel update against
    its own dimension, which should be comparable to it; absolute pose NEES is
    deliberately not reported, because the global position and yaw are the navigation
    frame's gauge and a NEES over them measures a frame convention rather than the
    filter.}
  \label{tab:rpe}
  \begin{tabular}{lcccc}
    \toprule
     & \textbf{2m} & \textbf{5m} & \textbf{10m} & \textbf{wheel NIS} \\
    \midrule
    VIO & 2.917 / 0.401 & 3.848 / 0.623 & 3.370 / 0.813 & -- \\
    true w. cal & 2.381 / 0.148 & 2.539 / 0.195 & 2.840 / 0.203 & 1.52 / 3 \\
    true wo. cal & 2.545 / 0.112 & 3.046 / 0.210 & 3.653 / 0.333 & 2.50 / 3 \\
    bad w. cal & 2.203 / 0.137 & 2.311 / 0.188 & 2.280 / 0.191 & 1.45 / 3 \\
    bad wo. cal & 2.582 / 0.161 & 2.755 / 0.268 & 2.725 / 0.421 & 3.51 / 3 \\
    \bottomrule
  \end{tabular}
\end{table}

